A Neighbourhood Framework for Resource-Lean Content Flagging

We propose a novel framework for cross-lingual content flagging with limited target-language data, which significantly outperforms prior work in terms of predictive performance. The framework is based on a nearest-neighbour architecture. It is a modern instantiation of the vanilla k-nearest neighbour model, as we use Transformer representations in all its components. Our framework can adapt to new source-language instances, without the need to be retrained from scratch. Unlike prior work on neighbourhood-based approaches, we encode the neighbourhood information based on query--neighbour interactions. We propose two encoding schemes and we show their effectiveness using both qualitative and quantitative analysis. Our evaluation results on eight languages from two different datasets for abusive language detection show sizable improvements of up to 9.5 F1 points absolute (for Italian) over strong baselines. On average, we achieve 3.6 absolute F1 points of improvement for the three languages in the Jigsaw Multilingual dataset and 2.14 points for the WUL dataset.

==> TACL_ Resource-Lean Content Flagging/introduction.tex <==
\section{Introduction}

Online content moderation is an increasingly important problem -- small-scale websites and large-scale corporations alike strive to remove harmful content from their platforms~\cite{vidgen-etal-2019-challenges,pavlopoulos-etal-2017-deeper,wulczyn2017ex}. 
This is partly in anticipation of proposed legislation, such as the \textit{Digital Service Act} \cite{digitalservicesact2020} in the EU and the \textit{Online Harms Bill} \cite{online_harm_bill} in the UK. Moreover, the lack of content moderation can have significant impact on businesses (e.g.,~Parler was denied server space),
%\footnote{\url{https://www.nbcnews.com/tech/tech-news/amazon-suspends-hosting-parler-its}\linebreak\url{-servers-citing-violent-content-n1253648}}), 
on governments (e.g.,~the U.S. Capitol Riots),
%\footnote{\url{https://www.cbsnews.com/news/capitol-riot-arrests-2021-02-27/}}), 
and on individuals, e.g., because hate speech is linked to self-harm \cite{jurgens-etal-2019-just}.

A key challenge when developing content moderation systems is the lack of resources for many languages (other than English). With this in mind, here we aim to create a content flagging model for a target language with limited annotated data by transferring knowledge from another dataset in a different language, for which a large amount of training data is available. 


Various approaches have been proposed in the literature to address the lack of enough training data in the target language. A popular approach is to fine-tune large-scale pre-trained multilingual language models such as XLM~\cite{lample2019cross}, XLM-R~\cite{conneau2020-xlm-roberta}, or mBERT~\cite{devlin2019bert} on the target dataset ~\cite{glavas-etal-2020-xhate, stappen2020cross}. In order to incorporate knowledge from the source dataset, a sequential adaptation technique can be used that first fine-tunes a multilingual language model (LM) on the source dataset, and then on the target dataset \cite{garg2020tanda}. There are also existing approaches for mixing the source and the target datasets \cite{shnarch2018will} in different proportions, followed by fine-tuning the multilingual language model on the resulting dataset. While sequential adaptation introduces the risk of forgetting the knowledge from the source dataset, such mixing methods are driven by heuristics that are effective, but not systematic. Crucially, as we argue in this paper, this is because they do not model the relationship between the source and the target datasets. Another problem arises if we consider that examples with novel labels can be added to the source dataset. This is a specifically pertinent issue for content moderation, as efforts to create new resources often lead to the introduction of new label inventories or taxonomies \cite{banko-etal-2020-unified}. In that case, model re-training becomes a requirement in order to be able to map the new label space to the output layer that is used for fine-tuning. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/conceptual_diagram_tacl.pdf}
    \caption{Conceptual diagram of our neighbourhood framework. The query is processed using run-time compute, while the neighbour vector is pre-computed.}
    \label{fig:conceptual_framework}
\end{figure}

We propose a Transformer-based $k$-Nearest Neighbour (\knnplus) framework,\footnote{We use a `+' superscript to indicate that our \knnplus framework is an improvement over the vanilla $k$-NN model.} a one-stop solution and a significant improvement over the vanilla $k$-NN model. Our framework addresses the above-mentioned challenges, which are not easy to solve via simple fine-tuning of pre-trained language models. Moreover, to the best of our knowledge, our framework is the first attempt to use $k$-NN for transfer learning for the task of abusive content detection. 


Given a query, which is a training or an evaluation data point from the target dataset, \knnplus\ retrieves its nearest neighbours using a language-agnostic sentence embedding model. Then, it constructs Transformer representations for the query and for its neighbours. After that, it computes interaction features, which are based on the interactions of the representations of the query with each of its neighbours.\footnote{We borrow the terminology from information retrieval, as the interactions between a query and a document in deep matching models are computed in a similar way~\citep{drmm}.}
 At training time, the interaction features are optimised using supervised training signals computed from the label of the query and the neighbour, so that the features indicate their level of agreement. 
 
 For example, if the query and its neighbour are both abusive, they agree on the labels. Thus, the interactions help the model learn a semantic similarity space in terms of labels. The framework further uses a self-attention mechanism to aggregate the interaction features from all the neighbours, and it uses the aggregated representation to classify the input query. This representation is computed from the interaction features and indicates the agreement of the query with the neighbourhood. As the predictions are made based on aggregated interaction features only, \knnplus can easily incorporate new examples with unseen labels without requiring re-training. The conceptual framework is shown in Figure~\ref{fig:conceptual_framework}; it is robust to neighbours with incorrect labels, as it can learn to disagree with them as part of its training process.

We instantiate two variants of our framework: Cross-Encoder (CE) \knnplus and Bi-Encoder (BE) \knnplus. The \deepcetwoknn concatenates the query and a neighbour, and passes that sequence through a Transformer to obtain interaction features. \deepbetwoknn computes representations of the query and of a neighbour by passing them individually through a Transformer, and computes interaction features from these representations. \deepbetwoknn is more efficient than \deepcetwoknn, but it does not yield the same performance gains. Both models outperform six strong baselines both in cross-lingual and in multilingual settings. Our contributions can be summarised as follows:


\begin{itemize}[noitemsep]

    \item We address cross-lingual transfer learning for content flagging with limited labelled data from the target language. 
    
    \item We demonstrate that neighbourhood methods, such as \knn{} are viable candidates for approaching content flagging. 
    
    \item We propose a novel framework, \knnplus{}, which, unlike a vanilla \knn{}, models the relationship between a data point and each of its neighbours to represent the neighbourhood, using language-agnostic Transformers.
    
    \item Our evaluation results on eight languages from two different datasets for abusive language detection show sizable improvements of up to 9.5 F1 points absolute (for Italian) over strong baselines. On average, we achieve improvements of 3.6 F1 points for the three languages in the Jigsaw Multilingual dataset, and of 2.14 F1 points on the WUL dataset. 

\end{itemize}


==> TACL_ Resource-Lean Content Flagging/macros.tex <==
\usepackage{soul}

\definecolor{Gray}{gray}{0.9}
\definecolor{Blue}{rgb}{0.8,0.85,1}
\definecolor{Red}{rgb}{1,0.85,0.8}
\definecolor{flagged}{RGB}{153, 0, 0}
\definecolor{neutral}{RGB}{56, 118, 29}

\newcommand{\rev}[1]{\textcolor{black}{#1}}

\newcommand{\crev}[1]{\textcolor{black}{#1}}
%  This is more for us not for them
\newcommand{\reviewerA}[1]{\textcolor{red}{#1}}
\newcommand{\reviewerB}[1]{\textcolor{purple}{#1}}
\newcommand{\reviewerC}[1]{\textcolor{orange}{#1}}

%  Extra one for deletions:
\newcommand{\revdel}[1]{\rev{\st{#1}}}

==> TACL_ Resource-Lean Content Flagging/proposed_model.tex <==
\section{\knnplus Framework}
\label{sec:proposed-model}

We present our \knnplus framework below.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.55\textwidth}
    \centering
        \includegraphics[width=\textwidth]{images/be_knn.pdf}
        \caption{Bi-Encoder \knn~(\deepbetwoknn) Variant.}
        \label{fig:be_knn}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ce_knn.pdf}
        \caption{Cross-Encoder \knn~(\deepcetwoknn) Variant.} 
        \label{fig:ce_knn}
    \end{subfigure}
    \caption{Two variants based on two encoding schemes used in our proposed \knnplus, where $\mathcal{M}_{feature}$ is the interaction feature computation model, $q$ is the query, and $c_i$ is a candidate neighbour. In the Bi-Encoder setup (Figure~\ref{fig:be_knn}), the query and each candidate are encoded separately using the same $\mathcal{M}_{feature}$ model. Afterwards, in order to obtain a joint vector representation for each query--candidate tuple, the query's representation ($rep_{q}$) is concatenated with each candidate's representation ($rep_{i}$) along with the absolute element-wise difference between the two. In the Cross-Encoder setting (Figure~\ref{fig:ce_knn}), the query and each candidate are passed through the $\mathcal{M}_{feature}$ model, which produces the joint vector representation ($rep_{i}$) for the query--candidate tuple. Finally, we pass each joint representation through (\emph{i})~a linear layer to predict the label agreement between the query and the candidate, and (\emph{ii})~a self-attention layer followed by a linear projection layer to predict the label of the example.}
    \label{fig:knn_plus}
\end{figure*}

\subsection{Problem Setting} 
\label{sec:problem_setting}

Our goal is to learn a content flagging model from source and target datasets in different languages with different label spaces -- see Figure~\ref{fig:conceptual_framework} for an illustration of our framework.

Formally, we assume access to a source dataset for content flagging, $D^s= \big\{(x_i^s, \vb{y}_i^s)\big\}_{i=1}^{n_s}$, where $x^s_i$ is a textual content and $\vb{y}_i^s \in \mathcal{Y}$. Further, a target dataset is given, $D^t = \big\{(x_{j}^t, y_{j}^t)\big\}_{j=1}^{n_t}$, where $y_j^t \in \{flagged, neutral\}$. $D^s$ is resource-rich, i.e., $n_s \gg n_t$, and label-rich, i.e., $|   \mathcal{Y}|>2$. The label space,  $\mathcal{Y} = \{hate, insult, \ldots, neutral\}$, of $D^s$ contains fine-grained labels for different levels of abusiveness along with the \emph{neutral} label. We convert the label space of $D^s$ to align it with the label space of $D^t$ as follows: $\mathcal{Y}^\prime = \{flagged \mid x \in \mathcal{Y}, x \neq neutral\}$. Note that this conversion is needed at training time to compute label agreement in our proposed neighbourhood framework. However, 
at inference time, a conversion of the label space of $D^s$ is not needed, as the label of an item from $D^t$ is predicted using the latent representations of the neighbours, rather than their labels. This process is described in more detail in Section \ref{sec:architecture}. 


\subsection{Why a Neighbourhood Framework?} 

\label{sec:motivation}
A vanilla \knn{} predicts a content label by aggregating the labels of $k$ similar training instances. To this end, it uses the content as a query to retrieve neighbours from the training instances. We hypothesise that this retrieval step can be performed in a cross-lingual transfer learning scenario. In our setting, the queries are target dataset instances, and we index the source dataset for retrieval. 

Note that the target instances could also be considered as neighbours for retrieval, but we exclude them, as the target dataset is small.   

For a vanilla \knn{}\ model, the queries and the documents are represented using lexical features, and thus the model suffers from the curse of dimensionality~\cite{knn_dimensionality}. Moreover, the prediction pipeline becomes inefficient if the source dataset is considerably larger than the target dataset, as is our case here~\cite{knn_efficiency}.
Finally, for a vanilla \knn{}, there is no straight-forward way to map between different languages for cross-lingual transfer.

We address these problems by using a Transformer-based multilingual representation space~\cite{feng2020language} that computes the similarity between two sentences expressed in different languages. We assume that efficiency issues are less critical here for two main reasons: (\emph{i})~retrieval using dense vector sentence embeddings has become significantly faster with recent advances~\cite{johnson2019billion}, and (\emph{ii})~the number of labelled source data examples is not expected to go beyond millions, because obtaining annotations for multilingual abusive content detection is costly and the annotation process can be very harmful for the human annotators as well~\cite{schmidt2017survey, waseem:2016, malmasi2018challenges, mathur2018detecting}. 

Even though multilingual language models can make the vanilla \knn{} model a viable solution for our problem, it is hard to make predictions with that model. Once a neighbourhood is retrieved, a vanilla \knn{} uses a majority voting scheme for prediction, as the example in Figure~\ref{fig:conceptual_framework} shows. Given a flagged Turkish query, our framework retrieves two \emph{neutral} and one \emph{flagged} English neighbours. Here, the majority voting prediction based on the neighbourhood is incorrect. The problem is this: \emph{A non-parametric vanilla \knn{} cannot make a correct prediction with an incorrectly retrieved neighbourhood}. Thus, we propose a learned voting strategy to alleviate this problem. 


\subsection{The Architecture of \knnplus}\label{sec:architecture}

We describe our \knnplus framework (shown in Figure~\ref{fig:knn_plus}), including the training and the inference procedures. The framework includes neighbourhood retrieval, interaction feature computation and aggregation, and a multi-task learning objective function for optimisation, which we describe in detail below.  

\paragraph{Neighbourhood Retrieval}
We construct a retrieval index $R$ from the given source dataset, $D^s = \big\{(x_i^s, \vb{y}_i^s)\big\}_{i=1}^{n_s}$. For each given example $x^s_i \in D^s$, we compute its dense vector representation, $\vb{x}^s_i = \mathcal{M}_{retriever}(x^s_i)$. Here, $\mathcal{M}_{retriever}$ is a multilingual sentence embedding model that we use for retrieval. There are several multilingual sentence embedding models that we could use as $\mathcal{M}_{retriever}$~\cite{10.1162/tacl_a_00288,reimers-gurevych-2020-making, chidambaram-etal-2019-learning,feng2020language}. In this work, we use LaBSE~\cite{feng2020language}, a strong multilingual sentence matching model, which has been trained with parallel sentence pairs from 109 languages. The model is trained on 17 billion monolingual sentences and 6 billion bilingual sentence pairs and it has achieved state-of-the-art performance for a parallel text retrieval task proposed by \citet{zweigenbaum-etal-2017-overview}.
We use $\vb{x}^s_i$ as a key, and we assign $(x_i^s, \vb{y_i}^s)$ as its corresponding value. Our retrieval index $R$ stores all the key-value pairs computed from the source dataset. 

Assume we have a training data point, $(x^t_j, y^t_j)  \in D^t$, from the target dataset. We consider the content $x^t_j$ as our query $q$, i.e., $q=x^t_j$. We compute a vector representation of the query,  $\vb{q} = \mathcal{M}_{retriever}(q)$. We use $\vb{q}$ to score each key, $\vb{x}^s_i$ of $R$ using cosine similarity, i.e.,~$cos(\vb{q}, \vb{x}^s_i)$.

We sort the items in $R$ in descending order of the scores of the keys, and we take the values of the top-$k$ items to construct the neighbourhood of $q$, $N_{q} = \{(c_1, l_1), (c_2, l_2), \ldots , (c_k, l_k)\}$. Thus, each neighbour is a tuple of a content and its label from the source dataset. We convert fine-grained neighbour labels to binary labels (\emph{flagged, neutral}) as described in Section~\ref{sec:problem_setting}, to align the label space with the target dataset. Nevertheless, the original fine-grained labels of the neighbours can be used to get an explanation at inference time as this is one of the core features of \knn-based models. However, our focus is on combining these models with Transformer-based ones. We leave the investigation of the explainability characteristics of \knnplus for future work.


\paragraph{Interaction Feature Modelling} 
As discussed in Section~\ref{sec:motivation}, the neighbourhood retrieval process might lead to prediction errors. Thus, we propose a learned voting strategy to mitigate this. Our proposed strategy depends on how $q$ relates to its neighbourhood $N_q$. To model this relationship, we compute the interaction features between $q$ and the content of its $j$-th neighbour, $c_j \in N_q$. We obtain a set of $k$ interaction features from $k$ neighbours, and we optimise them using query and neighbour labels.


Similarly to \citet{reimers-gurevych-2019-sentence}, we apply two encoding schemes to compute the interaction features: a \textbf{Cross-Encoder (CE)} and \textbf{Bi-Encoder (BE)}. Under our \knnplus framework, we refer to the schemes as \deepcetwoknn for CE, and \deepbetwoknn for BE. The \deepbetwoknn is computationally inexpensive, while the \deepcetwoknn is more effective. We provide a justification for this as we describe the schemes in the following paragraphs. 


For the \deepcetwoknn implementation (see Figure~\ref{fig:ce_knn}), we first form a set of query--neighbour pairs $S_{ce} = \{(q, c_1), (q, c_2), \ldots, (q, c_k)\}$ by concatenating $q$ with the content of each of its neighbours. Then, we obtain the output representation, $rep_j = \mathcal{M}_{feature}(q, c_j)$ of each $(q, c_j) \in S_{ce}$, from a pre-trained multilingual language model $\mathcal{M}_{feature}$. In this way, we create a set of interaction features, $I_{ce} = \{rep_1, rep_2, \ldots, rep_j\}$ from $q$ and its neighbourhood. Throughout this paper, the [CLS] token representation of $\mathcal{M}_{feature}$ is taken as its final output. We use varieties of implementations of $\mathcal{M}_{feature}$ in the experimentation. Figure~\ref{fig:ce_knn} shows how the interaction features are computed and optimised with a \deepcetwoknn.

Note that the feature interaction model $\mathcal{M}_{feature}$ is different from the neighbourhood retrieval one $\mathcal{M}_{retriever}$. We optimise interaction features from $\mathcal{M}_{feature}$, and we leave retrieval model optimisation for future work. 

For the \deepbetwoknn scheme (see Figure~\ref{fig:be_knn}), we obtain the output representations of $q$ and each of the neighbours individually from $\mathcal{M}_{feature}$. Given the representation of the query, $rep_q = \mathcal{M}_{feature}(q)$, and the representation of its $j^{th}$ neighbour, $rep_j = \mathcal{M}_{feature}(c_j)$, we model their interaction features by concatenating them along with their vector difference. The interaction features obtained for the $j$-th neighbour are $(rep_{q}, rep_j, |rep_{q} - rep_j|) $, and we construct a set of interaction features $I_{be}$ from all the neighbours of $q$. We use the vector difference $|rep_{q} - rep_j|$ along with the content vectors $rep_{q}$ and $rep_j$ following the work of \citet{reimers-gurevych-2019-sentence}. They trained a sentence embedding model using a Siamese neural network architecture with Natural Language Inference (NLI) data. They tried the following approaches to obtain features between the representations $u$ and $v$ of two sentences: $(u, v), (|u-v|), (u*v), (|u-v|, u*v), (u,v,u*v), (u,v,|u-v|), (u,v,|u-v|), (u*v)$. Their empirical analysis showed that $(u,v,|u-v|)$ works the best for NLI data, and thus we apply this in our framework. We plan to explore other options in future work.

Both the cross-encoder and the bi-encoder architectures were shown to be effective in a wide variety of tasks including Semantic Textual Similarity and Natural Language Inference. \citet{reimers-gurevych-2019-sentence} showed that a bi-encoder is much more efficient than a cross-encoder, and that bi-encoder representations can be stored as sentence vectors. Thus, once $\mathcal{M}_{feature}$ is trained, the vector representations $\mathcal{M}_{feature}(x_i^s)$ of each $x_i^s \in D^s$ can be saved along with the textual contents and label. Then, at inference time, only the representation of the query needs to be computed, which reduces the computation time from $k \times \mathcal{M}_{feature}$ to a constant time. Moreover, the model can easily adapt to new neighbours without the need for retraining. However, from an effectiveness perspective, the cross-encoder is usually a better option as it encodes the query and its neighbour jointly, thus enabling multi-head attention-based interactions among the tokens of the query and of the neighbour. 


\paragraph{Choice of $\mathcal{M}_{feature}$}

We explore two $\mathcal{M}_{feature}$ models for both the CE and the BE schemes: a pre-trained XLM-R model, which we will refer to as \modelxlmr, as well as an XLM-R model augmented with \emph{paraphrase} knowledge, which we will refer to as \modelpxlmr~\cite{reimers-gurevych-2020-making}. Sentence representations from XLM-R are not aligned across languages~\cite{ethayarajh-2019-contextual} and \modelpxlmr overcomes this problem. In particular, \modelpxlmr is trained to learn sentence semantics with parallel data from 50 languages. Moreover, the training process includes knowledge distillation from a Sentence BERT model~\cite{reimers-gurevych-2019-sentence} trained on 50 million English paraphrases. As such, we expect \modelpxlmr to outperform \modelxlmr, as it more accurately captures the semantics of the query and its neighbour sentences.
Note that there is work on producing better alignments of multilingual vector spaces \cite{zhao2020inducing}, which would allow us to consider a variety of pre-trained sentence representation models, but exploring this is outside the scope of this paper.

\paragraph{Interaction Features Optimisation} Given a query $q$ and its $j$-th neighbour, we obtain features $rep_j \in I_{ce}$ and $(rep_{q}, rep_j, |rep_{q} - rep_j|) \in I_{be}$ from $\mathcal{M}_{feature}$ for the \deepcetwoknn and \deepbetwoknn schemes, respectively. For both schemes, we optimise the interaction features to indicate whether a query and its neighbour have the same or different labels. We do this to later aggregate interaction features from all the neighbours of a query to model the overall agreement of the query with the retrieved neighbourhood. Our hypothesis is that understanding  individual neighbour-level agreement and aggregating it will allow us also to understand the neighbourhood.

We apply a fully connected layer with two outputs over the interaction features to optimise them. The outputs indicate the label agreement between $q$ and its $j$-th neighbour, $(c_j, l_j) \in N_q$. There is a label agreement if both $q$ and the $j$-th neighbour are flagged or are both neutral, i.e.,~$y_j^t = l_j$. We learn the label agreement using a binary cross-entropy loss $\mathcal{L}_{lal}$, which is computed using the output of a softmax layer for each example in a batch of training data. We refer to $\mathcal{L}_{lal}$ as label-agreement loss. In our implementation, a batch of data comprises a query and its $k$ neighbours. We provide more details about the training procedure in Section~\ref{sec:finetune}. 


Note that as our model predicts label agreement, it also indirectly predicts the label of the query and of the neighbour. In this way, it learns representations that separate flagged from the non-flagged examples. 

\paragraph{Interaction Features Aggregation}
The main reasons to use interaction features for label agreement is to predict whether $q$ should be flagged or not. In a vanilla \knn setup, there is no mechanism to back-propagate classification errors, as the only parameter to tune there is the hyper-parameter $k$. In our model, we propose to optimise the interaction features -- using a self-attention module -- to minimise the classification error with a fixed neighbourhood size $k$. To this end, we propose to aggregate the $k$ interaction features: $I_{ce}$ for \deepcetwoknn and $I_{be}$ for \deepbetwoknn. The aggregated representation captures global information, i.e.,~the agreement between the query and its neighbourhood, whereas the interaction features capture them locally. 

We use structured self-attention~\cite{lin2017structured} to capture the neighbourhood information. At first, we construct an interaction features matrix, $H \in \mathbb{R}^{k\times h}$ from the set of $k$ neighbours ($I_{ce}$ or $I_{be}$), where $h$ is the dimensionality of the interaction feature space. Then, we compute structured self-attention as follows:
\begin{align}
\vec{a} &=\operatorname{softmax}\left(W_{2} \tanh \left(W_{1} \mathbf{H}^T\right)\right)\\
			\mathbf{rep_i}&=\vec{a} \mathbf{H}
\end{align}%

Here, $W_{1} \in \mathbb{R}^{h_r \times h}$ is a matrix that encodes interactions between the representations and projects the interaction features into a lower-dimensional space, $h_r < h$, thus making the representation matrix $h_r \times k$ dimensional. We multiply another matrix $W_{2} \in \mathbb{R}^{1 \times h_r}$ by the resulting representation, and we apply softmax to obtain a probability distribution over the $k$ neighbours. Then, we use this probability distribution to produce an attention vector that linearly combines the interaction features to generate the neighbourhood representation $rep_{N_q}$, which we eventually use for classification. 

\paragraph{Classification Loss Optimisation} The aggregated interaction features, $rep_{N_q}$, are used as an input to a softmax layer with two outputs (\emph{flagged} or \emph{neutral}), which we optimise using a binary cross-entropy loss, $\mathcal{L}_{cll}$. We refer to $\mathcal{L}_{cll}$ as classification loss.

Optimising this loss means that the classification decision for a query is made by computing its agreement or disagreement with the neighbourhood as a whole. Our approach is a multi-task learning one, and the final loss is computed as follows: 
\begin{align}
\mathcal{L} = (1-\lambda) \times \mathcal{L}_{lal} + \lambda \times  \mathcal{L}_{cll}
\end{align}%


As both the classification and the label-agreement tasks aid each other, we adopt a multi-task learning approach. We balance the two losses using the hyper-parameter $\lambda$. The classification loss forces the model to predict a label for the query. As the model learns to predict a label for a query, it becomes easier for it to reduce the label agreement loss $\mathcal{L}_{lal}$. Moreover, as the model learns to predict label agreement, it learns to compute interaction features, which represent agreement or disagreement. This, in turn, helps to optimise $\mathcal{L}_{cll}$.

Note that, at inference time, our framework requires neither the labels of the neighbours for classification, nor a heuristic-based label-aggregation scheme. The classification layer makes a prediction based on the pooled representation from the interaction features, thus removing the need for any heuristic-based voting strategy based on the labels of the neighbours. Each individual interaction feature from the query and a neighbour captures the agreement between them as we optimise the features via the $L_{lal}$ loss. The opinion of the neighbourhood is captured using an aggregation of individual interaction features -- which is different from a vanilla \knn{} -- where neighbourhood opinion is captured using an individual neighbour label. As our aggregation is performed using a self-attention mechanism, we obtain a probability distribution over the interaction features that we can use to find the neighbour that influenced the neighbourhood opinion the most. We also know both the original and the converted label of the neighbour (see Section \ref{sec:problem_setting} for further details about the label space conversion). The original label of the neighbour could help us understand the prediction behind the query better. For example, if the query is flagged and the original label of the most influential neighbour is \emph{hate}, we could infer that the query is hate speech. However, we do not explore this direction in this paper, and we leave it as a future work.

==> TACL_ Resource-Lean Content Flagging/related_work.tex <==
\section{Related Work}
Below, we review recent work on abusive language detection and neighbourhood approaches.

\subsection{Abusive Content Detection}

Most approaches for abusive language detection use text classification models, which have been shown to be effective for related tasks such as sentiment analysis. This includes SVMs \cite{macavaney2019hate}, CNNs \cite{georgakopoulos2018convolutional, badjatiya_www19, agrawal2018deep}, LSTMs \cite{Arango:2019, agrawal2018deep},  BiLSTMs, with attention \cite{agrawal2018deep}, Capsule networks \cite{srivastava-etal-2018-identifying}, and fine-tuned Transformers \cite{glavas-etal-2020-xhate}. All these approaches focus on single data points, while we also model their neighbourhoods. See \cite{nakov2021detecting} for a recent survey of abusive language detection. 


Several papers studied the bias in hate speech detection datasets and criticised the use of within-dataset evaluations~\citep{Arango:2019, davidson, badjatiya_www19}, as this is not a realistic setting, and findings about generalisability based on such experimental settings are questionable. A more realistic and robust evaluation setting was investigated by \citet{glavas-etal-2020-xhate}, who showed the performance of online abuse detectors in a zero-shot cross-lingual setting. They fine-tuned several multilingual language models~\citep{devlin2019bert,lample2019cross,conneau2020-xlm-roberta,sanh2019distilbert,wang2020minilm} such as XLM-RoBERTa and mBERT on English datasets and observed how these models transfer to datasets in five other languages. Other cross-lingual abuse detection efforts include using Twitter user features for detecting hate speech in English, German, and Portuguese~\cite{fehn-unsvag-gamback-2018-effects}, cross-lingual embeddings~\cite{ranasinghe-zampieri-2020-multilingual}, and using multingual lexicon with deep learning~\cite{pamungkas-patti-2019-cross}. A lot of relevant research was also done as part of the OffensEval shared task at SemEval \cite{zampieri-etal-2019-predicting,zampieri-etal-2019-semeval,zampieri-etal-2020-semeval,rosenthal-etal-2021-solid}.

While understanding the performance of zero-shot cross-lingual models is interesting from a natural language understanding point of view, in reality, a platform willing to deploy an abusive language detection system can almost always provide some examples of malicious content for training. 

Thus, a few-shot or a low-shot scenario is more realistic, and we approach cross-lingual transfer learning from that perspective. We hypothesise that a nearest-neighbour model is a reasonable choice in such a scenario, and we propose several improvements over such a model. 


\subsection{Neighbourhood Models}

\knn\ models have been used for a number of
NLP tasks such as part of speech tagging~\citep{daelemans-etal-1996-mbt} and morphological analysis~\citep{bosch2007efficient}, among many others. Their effectiveness is rooted in the underlying similarity function, and thus non-linear models such as neural networks can bring additional boost to their performance. More recently, \citet{DBLP:conf/iclr/KaiserNRB17} used a similarly differentiable memory that is learned and updated during training and is then applied to one-shot learning tasks.  \citet{DBLP:conf/iclr/KhandelwalLJZL20} introduced $k$-NN retrieval for improving language modelling, which \citet{kassner-schutze-2020-bert} extended to question answering (QA). \citet{guu2020realm} proposed a framework for retrieval-augmented language modelling (REALM), showing its effectiveness on three Open QA datasets. \citet{NEURIPS2020_6b493230} explored a retrieval-augmented generation for a variety of tasks, including fact-checking and QA, among others. \citet{fan-etal-2021-augmenting} introduced a $k$-NN framework for dialogue generation using pre-trained embeddings enhanced by learning an alignment function for retrieval from a set of external multi-modal evidence sources. Finally, \citet{wallace-etal-2018-interpreting} proposed a deep $k$-NN approach for interpreting the predictions from a neural network for the task of natural language inference. 

All the above approaches use neighbours as additional information sources, but do not consider the interactions between the neighbours as we do. Moreover, there is no existing work on using deep \knn\ models for cross-lingual abusive content detection.


==> TACL_ Resource-Lean Content Flagging/tables/overall_results.tex <==
\begin{table*}[t]
	\centering
	\small
	\resizebox{1.00\textwidth}{!}{
	\setlength{\extrarowheight}{3pt}
		\begin{tabular}{r|lcccccccccc}            
		    \toprule

            &  & \multicolumn{3}{c}{\bf{Jigsaw Multilingual}} & \multicolumn{6}{c}{\bf{WUL}} \\ 
            
             \cmidrule(lr){3-5} \cmidrule(lr){6-11} 
             \# & \bf{Method} & ES & IT & TR & DE & EN & HR & RU & SQ & TR \\
            
            \midrule
            {1} & {Lexicon} & {35.8} & {40.5} & {34.0} & {70.9} & {70.6} & {63.9} & {63.6} & {58.2} & {71.8} \\
            2 & FastText & 55.3 & 47.2 & 64.2 & 74.2 & 72.7 & 58.9 & 74.2 & 65.9 & 72.5 \\ 
            
            \midrule
            
            3 & XLM-R Target & \underline{63.5} & 56.4 & 80.6 & 82.1 & 75.7 & 73.2 & 76.7 & 77.3 & 78.8 \\
            
            4 & XLM-R Mix-Adapt & \bf{64.2} & 58.5 & 76.1 &
            83.2 & \bf{93.9} & 87.3 & 82.1 & 86.2 & 86.0 \\ 
            
            5 & XLM-R Seq-Adapt & 60.5 & 58.3 & 81.2 &
            83.9 & 88.0 & 80.0 & 80.0 &  86.3 & 83.5 \\
            
            \midrule
            
            6 & LaBSE-kNN  & 44.7 & 48.5 & 66.0 &
            70.8 & 77.1 & 84.1 & 79.1 & 83.1 & 75.6 \\
            
            7 & Weighted LaBSE-kNN & 44.8 & 38.3 & 52.1 &
            71.7 & 85.4 & 82.4 & 79.5 & 83.7 & 81.0 \\

            \midrule
            
            \rowcolor{Red}
            
            8 & \deepcetwoknn + \modelxlmr & 58.9 & \underline{63.8} & 78.5 &
            80.4 & 83.8 & 86.2 & 77.6 & 83.5 & 85.4  \\
            
            \rowcolor{Red}
            
            9 & \deepcetwoknn + \modelpxlmr  & 59.4 & \bf{67.0} & \underline{84.4} &
            84.8 & 88.0 & 86.3 & 83.8 & 83.0 & 86.5 \\
       
            \rowcolor{Red}
            
            10 & \deepcetwoknn + \modelpxlmr $\rightarrow$ SRC  & 61.2 & 61.1 & \bf{85.0} &
            \bf{89.5} & \underline{92.3} & \bf{90.6} & 84.9 & \underline{89.5} & \underline{87.3} \\
            
            \rowcolor{Blue}
            
            11 & \deepbetwoknn + \modelxlmr  & 52.2 & 60.3 & 75.0 &
            81.6 & 80.8 & 77.9 & 78.0 & 79.6 & 79.6 \\
            
            \rowcolor{Blue}
            
            12 & \deepbetwoknn + \modelpxlmr & 58.8 & 56.6 & 80.6 &
            83.8 & 86.9 & 82.2 & \bf{86.9} & 84.9 & 83.7\\
            
            \rowcolor{Blue}
            13 & \deepbetwoknn + \modelpxlmr $\rightarrow$ SRC & 59.1 & 59.5 & 81.6 &
            \underline{88.7}  & 90.7 & \underline{87.6} & \underline{86.3} & \bf{90.2} & \bf{88.7} \\
            
            \bottomrule
        \end{tabular}
	}
	\caption{Comparison of F1 scores for the baselines and for our model variants. \deepbetwoknn and \deepcetwoknn indicate Bi-encoder and Cross-encoder schemes, respectively. SRC indicates that the model was further pre-trained with source \jigsawen, using data from it as both query and neighbours.}
	\label{tab:overall}
\end{table*}
